The Difference-of-Log-Normals Distribution: Properties, Estimation, and Growth

This paper describes the Difference-of-Log-Normals (DLN) distribution. A companion paper makes the case that the DLN is a fundamental distribution in nature, and shows how a simple application of the CLT gives rise to the DLN in many disparate phenomena. Here, I characterize its PDF, CDF, moments, and parameter estimators; generalize it to N-dimensions using spherical distribution theory; describe methods to deal with its signature ``double-exponential'' nature; and use it to generalize growth measurement to possibly-negative variates distributing DLN. I also conduct Monte-Carlo experiments to establish some properties of the estimators and measures described.

==> FigTab.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Figures
\clearpage

% DLN Examples
\RPprep{DLN Examples}{0}{0}{DLNexam}{%
    This figure presents examples of the DLN distribution. Panel (a) graphs the PDFs of the standard Normal, log-Normal, and DLN. Panel (b) graphs the PDFs of standard DLN with different correlation coefficients $\rho_{pn}$. Panel (c) presents the PDFs of a DLN with parameters $(3,2,2,2)$, common in practice, and varying correlation coefficients $\rho_{pn}$. Panel (c) presents the PDF for the range $\pm 10$, which is a significant truncation due to the long tails of this DLN. Panel (d) presents the same PDFs as Panel (c), but the x-axis is asinh-transformed, such that it spans the range sinh(-10) $\approx$ -11,000 to sinh(10) $\approx$ 11,000.
}
\RPfig{%
	\begin{tabular}{cc} 
		\subfigure[standard DLN, N, LN]{\includegraphics[width=3in]{Img/DLN_N_LN.pdf}} & 
		\subfigure[Std. DLN w/ corrs]{\includegraphics[width=3in]{Img/SDLN_corrs.pdf}} \\ \\
		\subfigure[DLN w/ corrs]{\includegraphics[width=3in]{Img/DLN_corrs.pdf}} &
		\subfigure[ADLN w/ corrs]{\includegraphics[width=3in]{Img/ADLN_corrs.pdf}} \\ \\
	\end{tabular}
}



% Estimator Monte Carlo 
\RPprep{Estimator Monte-Carlo experiments}{0}{1}{MC1}{%
    This figure presents results of estimator Monte-Carlo experiments. Panel (a) graphs the dependence of the correlation between the theoretical and empirical moments on sample size. Panel (b) graphs the dependence of moment bias on sample size. Panel (c) presents the distribution of (log of) the K-S statistic in the simulations. Panels (d)-(f) then present the ICDF of the (log) K-S, C-2, and A-D statistics, along with the fitted curves.
}
\RPfig{%
	\begin{tabular}{ccc} 
		\subfigure[Corr($\text{asinh}(\widehat{M}_i),\text{asinh}(M_i)$)] {\includegraphics[width=2.5in]{Img/Moment_Corr.pdf}} & 
		\subfigure[Median($\text{asinh}(\widehat{M}_i)-\text{asinh}(M_i)$)] {\includegraphics[width=2.5in]{Img/Moment_Bias.pdf}} & 
		\subfigure[PDF of log K-S statistic] {\includegraphics[width=2.5in]{Img/KS_PDF.pdf}} \\ \\
		\subfigure[ICDF of log K-S statistic]
		{\includegraphics[width=2.5in]{Img/KSfit.pdf}} &
		\subfigure[ICDF of log C-2 statistic]
		{\includegraphics[width=2.5in]{Img/C2fit.pdf}} &
		\subfigure[ICDF of log A-D statistic]
		{\includegraphics[width=2.5in]{Img/ADfit.pdf}} \\ \\
	\end{tabular}
}



% Growth Monte-Carlo
\RPprep{Growth Monte-Carlo experiments}{1}{0}{MC2}{%
    This figure presents results of growth Monte-Carlo experiments. Panels (a) and (b) graph the relation between the growth of a Normal RV and (a) generalized percentage growth d\%($Z_{t+1}$)=$\left(Z_{t+1} - Z_{t}\right/\left|Z_{t}\right|$; (b) log point growth dlog($Z_{t+1}$)=log($Z_{t+1}$)-log($Z_{t}$). Panels (c) and (d) graph the relation between the growth of a log-Normal RV and (c) dlog($Z_{t+1}$) ; (d) d\%($Z_{t+1}$). Panels (e) and (f) graph the relation between the growth of a DLN RV and (e) the DLN growth measure from Equation~\ref{eq:DLNGROWTH}, dDLN($Z_{t+1}$); (f) d\%($Z_{t+1}$).
}
\RPfig{%
	\begin{tabular}{cc} 
		\subfigure[N growth vs. d\%$^1$] {\includegraphics[width=2.5in]{Img/N_grow_per.pdf}} & 
		\subfigure[N growth vs. dlog$^2$] {\includegraphics[width=2.5in]{Img/N_grow_dlog.pdf}} \\ 
		\subfigure[LN growth vs. dlog] {\includegraphics[width=2.5in]{Img/LN_grow_dlog.pdf}} & 
		\subfigure[LN growth vs. d\%] {\includegraphics[width=2.5in]{Img/LN_grow_per.pdf}} \\ 		
		\subfigure[DLN growth vs. dDLN$^1$] {\includegraphics[width=2.5in]{Img/DLN_grow_dDLN.pdf}} & 
		\subfigure[DLN growth vs. d\%$^1$] {\includegraphics[width=2.5in]{Img/DLN_grow_per.pdf}} \\ 
	\end{tabular}
    \begin{flushleft}
    $^1$ For non-tiny initial values ($\left|Z_{t}\right|>1$) \\
	$^2$ For strictly positive and non-tiny initial values ($Z_{t}>1$ and $Z_{t+1}>0$) \\
    \end{flushleft}	
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tables
\clearpage

\RPprep{Estimator Monte Carlo Experiments}{0}{0}{MC1}{%
    This table presents results of estimator Monte-Carlo experiments with $N=70,000$ repetitions and $K=100,000$ observations drawn in each repetition. Panel (a) tests the moments estimators $\widehat{M}_i\ \ i\in\{1...5\}$ of Section~\ref{sec:Moms} vs. the actual moments $M_i$, conducting all analysis in asinh space. It reports the general accuracy corr($\text{asinh}(\widehat{M}_i),\text{asinh}(M_i)$); the bias median($\text{asinh}(\widehat{M}_i)-\text{asinh}(M_i)$) ; and the accuracy IQR($\text{asinh}(\widehat{M}_i)-\text{asinh}(M_i)$). Panel (b) reports similar statistics comparing the DLN parameter estimators of Section~\ref{sec:Estim} $\pmb{\widehat{\Theta}}$ and the actual parameters $\pmb{\Theta}$. Panel (c) reports the values of parameters a,b,c,d in the approximations $ICDF(p) = a\cdot\exp(b\cdot p) + c\cdot\exp(d\cdot p)$ for the ICDFs of the Kolmogorov-Smirnov, Chi-square, and Anderson-Darling test statistics for DLN RVs, as well as the approximation $R^2$.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrr}
    \toprule
	\textit{Panel (a): Moment estimators} & $\widehat{M}_1$ & $\widehat{M}_2$ & $\widehat{M}_3$ & $\widehat{M}_4$ & $\widehat{M}_5$ \\
    \midrule
    Correlation                 &  0.9997  &  0.9929 &  0.9282 &  0.8238 &  0.8478 \\
    Bias                        &  -0.0001 &  0.1092 & -0.0002 &  6.3410 & 0.0220 \\
    Accuracy                    &  0.0217  &  0.4785 &  3.4480 &  8.5609 & 32.0236 \\ \\
    
	\textit{Panel (b): Parameter estimators} & $\widehat{\mu}_p$ & $\widehat{\sigma}_p$ & $\widehat{\mu}_n$ & $\widehat{\sigma}_n$ & $\widehat{\rho}_{pn}$ \\
    \midrule
    Correlation                 &  0.9408 &  0.9619 &  0.9412 &  0.9623 &  0.9190 \\
    Bias                        & -0.0034 &  0.0019 & -0.0043 &  0.0019 & -0.0048 \\
    Accuracy                    &  0.0588 &  0.0251 &  0.0614 &  0.0259 &  0.0762 \\ \\

    \textit{Panel (c): ICDF approximations} & a & b & c & d & $R^2$ \\
    \midrule
    Kolmogorov-Smirnov          & 6.75e-7 &  0.1553 & -6.7520 & -0.0011 &  0.9976 \\
    Chi-square                  & 1.88e-8 &  0.1955 &  1.2080 &  0.0044 &  0.9920 \\
    Anderson-Darling            & 1.18e-5 &  0.1350 & -5.7070 & -0.0060 &  0.9900 \\
	\bottomrule
    \end{tabularx}
}



\RPprep{Growth Monte Carlo Experiments}{0}{0}{MC2}{%
    This table presents results of growth Monte-Carlo experiments with $N=10,000$ repetitions and $K=1,000$ observations simulated forward in each repetition. Panels (a), (b), and (c) present results for N, LN, DLN, respectively. Within each panel, I report correlations between the following measures of growth: $\epsilon_t$ the stochastic innovation underlying the growth at time $t$; $\epsilon_t/\left|Z_{t}\right|$ the relative stochastic innovation; d\%($Z_{t+1}$)=$\left(Z_{t+1} - Z_{t}\right/\left|Z_{t}\right|$ the generalized percentage growth; dlog($Z_{t+1}$)=log($Z_{t+1}$)-log($Z_{t}$) the log point growth; dDLN($Z_{t+1}$) the DLN growth formulation based on Equation~\ref{eq:DLNGROWTH}.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Flllll}
    \toprule
	\textit{Panel (a): N} & $\epsilon_t$ & $\epsilon_t/\left|Z_{t}\right|$ & d\%($Z_{t+1}$) & dlog($Z_{t+1}$) & \\
    \midrule
    $\epsilon_t$ 
    & 1.000 & 0.010 & 0.009 & 0.659$^{1}$ & \\
    $\epsilon_t/\left|Z_{t}\right|$ 
    & 0.380$^{2}$ & 1.000 & 0.973 & 0.031$^{1}$ & \\
    d\%($Z_{t+1}$) 
    & 0.357$^{2}$ & 0.960$^{2}$ & 1.000 & 0.033$^{1}$ & \\
    dlog($Z_{t+1}$) 
    & 0.712$^{2}$ & 0.590$^{2}$ & 0.617$^{2}$ & 1.000 & \\ \\

	\textit{Panel (b): LN} & $\epsilon_t$ & $\epsilon_t/\left|Z_{t}\right|$ & d\%($Z_{t+1}$) & dlog($Z_{t+1}$) & \\
    \midrule
    $\epsilon_t$ 
    & 1.000 & 0.023$^{1}$ & 0.269$^{1}$ & 0.931$^{1}$ & \\
    $\epsilon_t/\left|Z_{t}\right|$
    & 0.644$^{2}$ & 1.000 & 0.097$^{1}$ & 0.023$^{1}$ & \\
    d\%($Z_{t+1}$) 
    & 0.381$^{2}$ & 0.363$^{2}$ & 1.000 & 0.295$^{1}$ & \\
    dlog($Z_{t+1}$) 
    & 0.929$^{2}$ & 0.620$^{2}$ & 0.381$^{2}$ & 1.000 & \\ \\

	\textit{Panel (c): DLN} & $\widehat{\epsilon}_t^3$ & $\widehat{\epsilon}_t/\left|Z_{t}\right|^3$ & d\%($Z_{t+1}$) & dlog($Z_{t+1}$) & dDLN($Z_{t+1}$) \\
    \midrule
    $\widehat{\epsilon}_t^3$ 
    & 1.000 & 0.000$^{1}$ & 0.000$^{1}$ & 0.038$^{1}$ & 0.000$^{1}$ \\
    $\widehat{\epsilon}_t/\left|Z_{t}\right|^3$
    & 0.043$^{2}$ & 1.000 & 0.652 & 0.022$^{1}$ & 0.944 \\
    d\%($Z_{t+1}$) 
    & 0.009$^{2}$ & 0.464$^{2}$ & 1.000 & 0.016$^{1}$ & 0.645 \\
    dlog($Z_{t+1}$) 
    & 0.057$^{2}$ & 0.739$^{2}$ & 0.397$^{2}$ & 1.000 & 0.023$^{1}$ \\
    dDLN($Z_{t+1}$)
    & 0.040$^{2}$ & 0.931$^{2}$ & 0.455$^{2}$ & 0.797$^{2}$ & 1.000 \\ \\
    \bottomrule
    \end{tabularx}
    \begin{flushleft}
    $^1$ For strictly positive values ($Z_{t}>0$ and $Z_{t+1}>0$) \\
	$^2$ For strictly positive and non-tiny initial values ($Z_{t}>1$ and $Z_{t+1}>0$) \\
	$^3$ For DLN, I define $\widehat{\epsilon}_t = \left(Z_t^p\cdot\epsilon_t^p - Z_t^n\cdot\epsilon_t^n\right)$ and $Z_t = Z_t^p - Z_t^n$
    \end{flushleft}
}



\RPprep{Approximation Monte Carlo Experiments}{0}{0}{MC3}{%
    This table presents results of approximation Monte-Carlo experiments with $N=25,000$ repetitions and $K=100,000$ observations drawn in each repetition. For each compound distribution tested, Panel (a) reports the share of observations rejected as being DLN at the 1\%, 5\%, and 10\% confidence levels using each of the three distributional tests K-S, C-2, and A-D. Panels (b) and (c) present the (5,10,50)$^{th}$ percentiles of the test statistics and their accompanying p-values, respectively, across all Monte-Carlo runs for each compound distribution.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrrr}
    \toprule
    & \multicolumn{3}{c}{K-S} & \multicolumn{3}{c}{C-2} & \multicolumn{3}{c}{A-D} \\
	\textit{Panel (a): rejected} & \multicolumn{1}{c}{1\%} & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c}{1\%} & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c}{1\%} & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} \\
    \midrule
    DLN + DLN   & 0.007 & 0.076 & 0.337 & 0.007 & 0.104 & 0.334 & 0.009 & 0.082 & 0.355 \\
    DLN * LN    & 0.101 & 0.377 & 0.539 & 0.111 & 0.408 & 0.538 & 0.084 & 0.378 & 0.549 \\
    DLN / LN    & 0.129 & 0.375 & 0.521 & 0.148 & 0.385 & 0.522 & 0.117 & 0.370 & 0.515 \\
    DLN * N     & 0.001 & 0.148 & 0.690 & 0.001 & 0.385 & 0.753 & 0.001 & 0.178 & 0.668 \\
    LN * N      & 0.000 & 0.070 & 0.324 & 0.000 & 0.080 & 0.270 & 0.000 & 0.086 & 0.353 \\ \\
    
	\textit{Panel (b): stats} & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c}{50\%} & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c}{50\%} & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c}{50\%} \\
    \midrule
    DLN + DLN   & 0.002 & 0.002 & 0.004 & 3.910 & 4.279 & 9.975 & 0.011 & 0.025 & 0.209 \\
    DLN * LN    & 0.001 & 0.002 & 0.008 & 3.349 & 3.855 & 32.59 & 0.006 & 0.009 & 1.068 \\
    DLN / LN    & 0.001 & 0.001 & 0.007 & 3.441 & 3.864 & 22.28 & 0.006 & 0.009 & 0.707 \\
    DLN * N     & 0.002 & 0.002 & 0.009 & 4.170 & 4.657 & 56.31 & 0.011 & 0.018 & 1.358 \\
    LN * N      & 0.001 & 0.001 & 0.002 & 3.233 & 3.660 & 5.321 & 0.008 & 0.010 & 0.042 \\ \\
    
	\textit{Panel (c): p-vals} & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c}{50\%} & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c}{50\%} & \multicolumn{1}{c}{5\%} & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c}{50\%} \\
    \midrule
    DLN + DLN   & 0.042 & 0.055 & 0.136 & 0.035 & 0.047 & 0.138 & 0.040 & 0.053 & 0.132 \\
    DLN * LN    & 0.000 & 0.010 & 0.082 & 0.000 & 0.007 & 0.073 & 0.001 & 0.013 & 0.080 \\
    DLN / LN    & 0.000 & 0.002 & 0.092 & 0.000 & 0.002 & 0.087 & 0.000 & 0.007 & 0.091 \\
    DLN * N     & 0.041 & 0.046 & 0.072 & 0.030 & 0.034 & 0.057 & 0.039 & 0.046 & 0.074 \\
    LN * N      & 0.044 & 0.058 & 0.238 & 0.047 & 0.056 & 0.315 & 0.040 & 0.055 & 0.247 \\
	\bottomrule
    \end{tabularx}
}

